APQ: Joint Search for Network Architecture, Pruning and Quantization Policy

We present APQ for efficient deep learning inference on resource-constrained hardware. Unlike previous methods that separately search the neural architecture, pruning policy, and quantization policy, we optimize them in a joint manner. To deal with the larger design space it brings, a promising approach is to train a quantization-aware accuracy predictor to quickly get the accuracy of the quantized model and feed it to the search engine to select the best fit. However, training this quantization-aware accuracy predictor requires collecting a large number of quantized <model, accuracy> pairs, which involves quantization-aware finetuning and thus is highly time-consuming. To tackle this challenge, we propose to transfer the knowledge from a full-precision (i.e., fp32) accuracy predictor to the quantization-aware (i.e., int8) accuracy predictor, which greatly improves the sample efficiency. Besides, collecting the dataset for the fp32 accuracy predictor only requires to evaluate neural networks without any training cost by sampling from a pretrained once-for-all network, which is highly efficient. Extensive experiments on ImageNet demonstrate the benefits of our joint optimization approach. With the same accuracy, APQ reduces the latency/energy by 2x/1.3x over MobileNetV2+HAQ. Compared to the separate optimization approach (ProxylessNAS+AMC+HAQ), APQ achieves 2.3% higher ImageNet accuracy while reducing orders of magnitude GPU hours and CO2 emission, pushing the frontier for green AI that is environmental-friendly. The code and video are publicly available.

==> bitops.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{bitops_1.png}
    \vspace{-10pt}
    \caption{Comparison with quantized model under BitOps constraint. Our model achieves 0.5\% accuracy boost (from 74.6\% to 75.1\%) compared models searched by single path one-shot while occupies half of BitOps. Also, the accuracy of our model is the same level as 8-bit version ResNet-34 model (75.0\%) while saving 8\times BitOps.}
    \vspace{-10pt}
\label{fig:bitops}
% \end{figure}
\end{wrapfigure}

==> compare_with_seq.tex <==
% \begin{figure}[t]
\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{compare_with_sequential.png}
    \caption{Comparison with \textit{sequentially designed} mixed-precision models searched by AMC and HAQ~\citep{cai2019proxylessnas,he2018amc,wang2019haq} under latency constraints. Our end-to-end designed model while achieving better accuracy than sequentially designed models. }
\label{fig:compare_with_seq}
\end{wrapfigure}
% \end{figure}


==> packages.tex <==
% basic
\usepackage{color,xcolor}
\usepackage{epsfig}
\usepackage{graphicx}

% figure and table
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
% \usepackage{subcaption} % issues a warning with CVPR/ICCV format

% font and character
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}

% layout
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

% ref
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=blue]{hyperref}
\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}
\usepackage{url}

% misc
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{enumerate}
% \usepackage{todonotes} % conflict with CVPR/ICCV format

\usepackage{titlesec}

==> tmp.tex <==


\begin{comment}
\subsection{Ablation Study on Mixed Quantization and Training Data}
\myparagraph{Fixed Precision v.s. Mixed Precision.}
\begin{wraptable}{r}{.25\linewidth}
\setlength{\tabcolsep}{2.5pt}
\centering
%\small
\begin{tabular}{l | c | c }
    \hline
    Model & Latency & Top1 (\%) \\
    \hline
    FP 8-bit & 15.35ms & 74.99 \\
    MP (Ours) & 15.20ms & 75.11  \\
    \hline
    \hline
	Model & Energy & Top1 (\%) \\
    \hline
    FP 8-bit & 15.88mJ & 74.63  \\
    FP 8-bit & 17.08mJ  & 74.98  \\
    MP (Ours) & 14.13mJ & 74.90 \\
    \hline
\end{tabular}
\caption{elastic bits}
\label{tab:elastic_bits}
\end{wraptable}
To verify the benefit of mixed precision optimization for our co-design method, we search for fixed precision model by forcing evolution only generate 8-bit quantization policy. As shown in \tianzhe{ref table}, we can see that mixed precision model either enjoys higher accuracy with similar efficiency constraints (0.12\% and 0.30\% accuracy boost for latency and energy consumption, respectively) or achieve the same level of accuracy with less resource consumption (from 17.08mJ to 15.87mJ for energy).

\myparagraph{Different Data to Train Predictor.}
\begin{wraptable}{r}{.45\linewidth}
\setlength{\tabcolsep}{2.5pt}
\centering
%\small
\vspace{-10pt}
\begin{tabular}{l | c | c }
    \hline
    Model & Constraint & Top1 (\%) \\
    \hline
    Proxyless & - & 74.20 \\
    \hline
    Mix5k & BitFLOPs & 73.42 \\
    Mix5k & Latency & 73.37  \\
	Mix5k & Energy & 73.53 \\
    \hline
    Mix5k + 8-bit & Latency & 74.83  \\
    Mix5k + 8-bit & Energy  & 74.90  \\
    \hline
\end{tabular}
\caption{empty.}
\label{tab:elastic_bits}
\end{wraptable}
In Table \tianzhe{ref table}, we show the different predictors's performance. We visualize two structure of the searched architecture and quantization policy in Figure \tianzhe{ref visual}. We can observe that for larger models, 8-bit data can guide the evolution searcher to seek for models with higher bits. It is also worth noticing that the trade between architecture's depth and bit width (from deeper to shallower, from lower bits to higher bits) helps to boost the accuracy.

\end{comment}

==> transfer_rebuttal.tex <==
% \begin{figure}[t]
\begin{wrapfigure}{r}{0.2\textwidth}
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{transfer_rebutal_1.pdf}
    \caption{The relationship between the performance of the accuracy predictor and number of data points.}
\label{fig:transfer_rebuttal}
% \vspace{-10pt}
\end{wrapfigure}
% \end{figure}


